Demystifying Orthogonal Monte Carlo and Beyond

Orthogonal Monte Carlo (OMC) is a very effective sampling algorithm imposing structural geometric conditions (orthogonality) on samples for variance reduction. Due to its simplicity and superior performance as compared to its Quasi Monte Carlo counterparts, OMC is used in a wide spectrum of challenging machine learning applications ranging from scalable kernel methods to predictive recurrent neural networks, generative models and reinforcement learning. However theoretical understanding of the method remains very limited. In this paper we shed new light on the theoretical principles behind OMC, applying theory of negatively dependent random variables to obtain several new concentration results. We also propose a novel extensions of the method leveraging number theory techniques and particle algorithms, called Near-Orthogonal Monte Carlo (NOMC). We show that NOMC is the first algorithm consistently outperforming OMC in applications ranging from kernel methods to approximating distances in probabilistic metric spaces.

==> additional.tex <==
\section{Extra material not included in main}
\label{sec:additional}

Let's consider $F_f(Z)=E_{\omega \in \mathcal{D}}[f(|\omega^T Z|)]$ where we assume $f: \mathcal{R}^{+} \mapsto \mathcal{R}$ can be expressed as Taylor series expending at zero with remaining term satisfying $\lim_{N \to \infty} R_N(x)=0$. The standard Monte Carlo estimator samples independently $\omega_i^{iid} \sim \mathcal{D}$, and then averages these samples over $i$: $\hat{F}_m^{iid}(Z)=\frac{1}{m} \sum_{i=1}^m f(|{\omega_i^{iid}}^T Z|)$, while the orthogonal estimator samples $\omega_i^{ort} \bot \omega_j^{ort}, \forall i \neq j $, and then averages over $i$: $\hat{F}_m^{ort}(Z)=\frac{1}{m} \sum_{i=1}^m f(|{\omega_i^{ort}}^T Z|)$. These orthogonal vectors can be constructed by performing Gram-Schimidt orthogonalization and then renormalizing the rows such that the length of the renormalized row is sampled from the
distribution from which $\Vert \omega_i^{iid} \Vert s$ are sampled. Both of these two estimators are trivially unbiased.

Now, let's explain how to utilize properties from negative association to prove that orthogonal random features can achieve better strong concentration bound than independent random features. 

Firstly, by applying Markov Inequality to some monotone functions, we can derive the following lemma.

\begin{lem} [Extended Markov Inequality] \label{Lem_ExtendedMarkovInequality} 
If $D(X)$ is a non-increasing and non-negative function for all $X \geq 0$, and $I(X)$ is a non-decreasing and non-negative function for all $X \geq 0$. Then $\forall X \geq 0, \forall k > 0 $, we have:
$$ P(X \geq k) = P(I(X)\geq I(k)) \leq \frac{E[I(X)]}{I(k)}$$
$$ P(X \leq k) = P(D(X)\geq D(k)) \leq \frac{E[D(X)]}{D(k)}$$
\end{lem}

We can apply Lemma \ref{Lem_ExtendedMarkovInequality} to our problem to get the concentration bound
$P( \hat{F}_{m} \geq a)\leq \frac{E[I(\hat{F}_{m}]}{I(a)} $ and 
$P( \hat{F}_{m} \leq a)\leq \frac{E[D(\hat{F}_{m}]}{D(a)} $ hold for both independent samples $\hat{F}_{m}^{iid}$ and orthogonal samples $\hat{F}_{m}^{ort}$, and $\forall a > 0$. If the orthogonal samples have better concentration bound than iid samples, then we should have
$ {E[I(\hat{F}^{ort}_{m})]} \leq {E[I(\hat{F}^{iid}_{m})]} $ and 
$ {E[D(\hat{F}^{ort}_{m})]} \leq {E[D(\hat{F}^{iid}_{m})]} $.

As for the specific form of $D(X)$ and $I(X)$, we can use exponential functions in order to transform the products of $m$ samples into summations. So we define $I(x)=\mathrm{e}^{\theta mx}$ and $D(x)=\mathrm{e}^{-\theta mx}$, where $\theta \geq 0$. Since $\hat{F}_{m}=\frac{1}{m}\sum_{i=1}^{m}X_{i}$, the equivalent inequality we need to prove can be written as
$ E[ \mathrm{e}^{ \theta\sum_{i=1}^{m}X_{i}^{ort} } ] \leq E[ \mathrm{e}^{ \theta \sum_{i=1}^{m}X_{i}^{iid} } ] = \prod_{i=1}^{m} E[\mathrm{e}^{\theta X_{i}^{iid} } ] $, and $ E[ \mathrm{e}^{ -\theta\sum_{i=1}^{m}X_{i}^{ort} } ] \leq E[ \mathrm{e}^{- \theta \sum_{i=1}^{m}X_{i}^{iid} } ] = \prod_{i=1}^{m} E[\mathrm{e}^{-\theta X_{i}^{iid} }]$.
If we combine these two inequalities, then we actually need to prove that
$ E[ \mathrm{e}^{ \lambda \sum_{i=1}^{m}X_{i}^{ort} } ] \leq \prod_{i=1}^{m} E[\mathrm{e}^{\lambda X_{i}^{iid} } ]$, Where $\lambda$ can take both positive and negative values.

Next, we first deviate from our proof by introducing the concepts of negative association (NA) and negative dependence (ND) from \cite{Wajc217,Joag-Dev183}, and then prove that $X_1^{ort},…,X_n^{ort}$ satisfy ND.

\begin{definition}[Negative Association (NA)] \label{Def_NA} 
A set of random variables $X_1,…,X_n$ is said to be negatively associated (NA) if for any two disjoint index sets $I,J \subseteq [n]$, and two functions $f and g$ either both non-decreasing or both non-increasing, it holds: $ E( f(X_i:i\in I) g(X_j:j\in J) ) \leq E(f(X_i:i\in I)) E(g(X_j:j\in J)) $ 
\end{definition}

\begin{lem} \label{Lem_appendix2}
Let $I_1,...,I_n$ be disjoint subsets of $\{1,...,k\}$ and $f_1,…,f_n$ be non-decreasing (non-increasing) positive functions. Then $X_1,…,X_k$ NA implies:
$$ E[\prod_{i=1}^{n} f_i(X_j:j\in I_i)] \leq \prod_{i=1}^n E[f_i(X_j: j \in I_i )]  $$
\end{lem}


Lemma \ref{Lem_NA_ExpectationProductInequality} can be proved by Definition 1 by induction. 
For $k=2$, we have already know it from Definition \ref{Def_NA}.
Assume that this holds for $k=m-1$. $ E[\prod_i^{m-1} f_i(X_j:j\in I_i)] \leq \prod_i^{m-1} E[f_i(X_j: j \in I_i )] $
For $k=m$, since the product of two monotone non-decreasing functions will also be monotone non-decreasing, so we can define $ f_{1:m-1} = \prod_i^{m-1} E[f_i(X_i: i \in I_i )] $, which will still be a monotone non-decreasing function defined on the union of the index sets of $X_1,…,X_{m-1}$, and this union set is also disjoint with the index set formed by $X_m$. And by using Definition \ref{Def_NA} and the assumption we made in the case $k=m-1$, Lemma \ref{Lem_NA_ExpectationProductInequality} can be proved. 

\begin{corollary} \label{Cor_NA_ProbabilityInequality}
If $X_1,…,X_n$ are NA random variables, then for any set of values $x_1,…,x_n$ and disjoint subsets $I,J \subseteq [n]$, it holds:
$ P(X_i \geq x_i, \forall i \in I \cup J ) \leq P(X_i \geq x_i, \forall i \in I) P(X_j \geq x_j, \forall j \in J) $, and 
$ P(X_i \leq x_i, \forall i \in I \cup J ) \leq P(X_i \leq x_i, \forall i \in I) P(X_j \leq x_j, \forall j \in J) $.
\end{corollary}


The first inequality in \ref{Cor_NA_ProbabilityInequality} can be proved by taking function $f$ and $g$ to be indicator functions $f(X_i:i\in I)=1\{X_i\geq x_i\}$ and $g(X_j:j\in J)=1\{X_j \geq x_j\}$. The second equation can be derived similarly by taking the indicator function in the other direction.

Now, let’s come back and understand how can we use these definitions and lemmas in our problem. And for clarity, we include another concept Negative Dependent (ND), which is a special case of Negative Associated we mentioned above.

\begin{definition}[Negative Dependence (ND)] \label{Def_ND}
Random variables $X_1,…,X_n$ are said to be negatively dependent if both of the following two inequalities holds for any $x_1,…,x_n \in R$
$$ P( \bigcap_i X_i \geq x_i ) \leq \prod_i P(X_i \geq x_i) $$ 
$$ P( \bigcap_i X_i \leq x_i ) \leq \prod_i P(X_i \leq x_i)  $$
\end{definition}

Definition \ref{Def_ND} follows by simply taking the disjoint index set of $X_1,…,X_n$ as $1,…,n$ in Corollary \ref{Cor_NA_ProbabilityInequality}. This definition is also stated as Marginal probability Bounds \cite{Wajc217}.

With such definition, we can derive some nice properties that will be used latter \cite{Rita208}.

\begin{lem} \label{Lem_ND_2points}
Let $X_1,…,X_n$ be negatively dependent random variables, then:
\begin{itemize}
  \item If $f_1,…,f_n$ is a sequence of measurable functions which are all monotone non-decreasing (or all are monotone non-increasing), then $f_1(X_1),…,f_n(X_n)$ are also negatively dependent random variables.
  \item $E[X_1…X_n ] \leq E[X_1]…E[X_n]$, provided the expectation exist.
\end{itemize}
\end{lem}

The first point follows by applying Definition \ref{Def_ND} in the following way:
If  $f_1,…,f_n$ are all monotone non-decreasing functions, then
$ P( \bigcap_{i=1}^n (f(X_i)\leq f(x_i)) ) = P( \bigcap_{i=1}^n (X_i\leq x_i) ) \leq 
\prod_{i=1}^n P(X_i \leq x_i) = \prod_{i=1}^n P(f(X_i) \leq f(x_i)) $, and 
$ P( \bigcap_{i=1}^n (f(X_i)\geq f(x_i)) ) = P( \bigcap_{i=1}^n (X_i\geq x_i) ) \leq 
\prod_{i=1}^n P(X_i \geq x_i) = \prod_{i=1}^n P(f(X_i) \geq f(x_i)) $. We can also prove this similarly if $f_1,…,f_n$ are all monotone non-increasing functions.

The LFS of the second point can be written as 
$ E[X_1...X_n] = \int\int...\int P( \bigcap_{i=1}^n(X_i\geq x_i))dx_1dx_2...dx_n $,
while the RHS equals to 
$ E[X_1]...E[X_n] = \int P(X_1\geq x_1)dx_1 ... \int P(X_n\geq x_1)dx_n = \int\int...\int \prod_{i=1}^n P(X_i\geq x_i) dx_1dx_2...dx_n $,
and the inequality follows since $P( \bigcap_{i=1}^n(X_i\geq x_i))\leq P(X_i\geq x_i)$.


\begin{lem} \label{Lem_ND_ExpectationProduct}
Let $X_1,…,X_n$ be negatively dependent random variables, then:
$$  E[\exp(\lambda \sum_{i=1}^m X_i)] \leq \prod_{i=1}^m E[e^{\lambda X_i}]  $$
\end{lem}


Firstly, by applying the first point in Lemma \ref{Lem_ND_2points}, we know that $f_1(X_1),…,f_n(X_n)$ are also negatively dependent random variables. 
Then by applying the second point in Lemma \ref{Lem_ND_2points}, $E[f_1(X_1 )…f_n(X_n)] \leq E[f_1(X_1)]…E[f_n(X_n)] $
If $ \lambda \geq 0$, then we can take a non-decreasing function $ f_i(X_i) = e^{\lambda X_i}$ for each $i$, and the inequality in this lemma holds. 
Similarly, if $ \lambda \leq 0$, then we can take a non-increasing function $f_i(X_i) = e^{\lambda X_i}$, and the inequality will also holds. Actually, we say that $X_1,...X_n$ are acceptable if the inequality in lemma \ref{Lem_ND_2points} holds for any real $\lambda$ \cite{Rita208}. And NA implies acceptability if the Laplace transforms $E[e^{\lambda X_i}]$ are finite for all $i$.

We notice that the inequality in Lemma \ref{Lem_ND_ExpectationProduct} is exactly the relationship we want to prove for orthogonal random features. Therefore, our next step is to prove that orthogonal random features are negatively dependent, which is consistent with our intuition.



\begin{lem} \label{Lem_abs_ort}
$\vert{\omega_1^{ort}}^T Z\vert,...,\vert{\omega_n^{ort}}^T Z\vert$ are negatively dependent.
\end{lem}

From the definition of negative dependence, what we need to prove is
$ P( \bigcap_i (\vert{w_i^{ort}}^T Z\vert \leq \tilde{x}_i) ) \leq \prod_i P(\vert{w_i^{ort}}^T Z\vert \leq \tilde{x}_i) $, and $ P( \bigcap_i (\vert{w_i^{ort}}^T Z\vert \geq \tilde{x}_i) ) \leq \prod_i P(\vert{w_i^{ort}}^T Z\vert \geq \tilde{x}_i) $, where we use $ \tilde{x}_i$  to represent a different value than the original $x_i$, which should be $f^{-1}(x_i)$. We will illustrate how to prove the first inequality here since the other can be proved accordingly.

Firstly, we can decompose $w_i^{ort}=v_i l_i$, where $v_i^{ort}$ has unit length, and $l_i$ is taken independent from $v_i^{ort}$, which represents the length scalar.
So we need to prove 
$ P( \bigcap_i (\vert{v_i^{ort}}^T Z\vert \leq \frac{\tilde{x}_i}{l_i} ) ) \leq \prod_i P(\vert{v_i^{orhttps://www.overleaf.com/project/5e1343de08771b000145df67t}}^T Z\vert \leq \frac{\tilde{x}_i}{l_i}) $.

But actually since negatively dependence should holds for any $x_i \in R$, so it actually does not matters which scalar we use in the right hand side of each part of the probability inequality. So we will continue to use $x_i$ instead of $\frac{\tilde{x}_i}{l_i}$  in the following proof.

Proof for the cases when $x_j\geq 1$ or $x_j\leq 0$ is trivial, so we will only concentrate on the case when $0< x_j < 1$. Here, we can use a second trick for distribution transformation. We regard $v_1$, $v_2$, ..., $v_n$ as fixed, and $Z$ as a random rotation vector. Furthermore, we assume $\Vert Z\Vert_2=1$ for simplicity. Then the distribution of $\vert{v_i^{ort}}^T Z\vert$ will be equivalent to $e_1^T \frac{\vert g \vert}{{\Vert g \Vert}_2}=\frac{g_i}{{\Vert g \Vert}_2}$, where $g$ is a gaussian vector, and $g_i$ is the length of projection onto the $i^{th}$ coordinate.

So we need to prove $ P( \bigcap_i (\frac{g_i}{{\Vert g \Vert}_2}\leq x_i) ) \leq \prod_i P(\frac{g_i}{{\Vert g \Vert}_2}\leq x_i) $.
From the rule of conditional probability, the LFS can be transformed to $ P(\frac{g_1}{{\Vert g \Vert}_2}\leq x_1)P(\frac{g_2}{{\Vert g \Vert}_2}\leq x_2 \vert \frac{g_1}{{\Vert g \Vert}_2}\leq x_1)P(\frac{g_3}{{\Vert g \Vert}_2}\leq x_3 \vert (\frac{g_1}{{\Vert g \Vert}_2}\leq x_1)\cap (\frac{g_2}{{\Vert g \Vert}_2}\leq x_2) )... $. Therefore, it’s obvious that we only need to prove $P(\frac{g_i}{{\Vert g \Vert}_2}\leq x_i \vert \bigcap_{j=1}^{i-1} (\frac{g_j}{{\Vert g \Vert}_2}\leq x_j) ) \leq P(\frac{g_i}{{\Vert g \Vert}_2}\leq x_i)$ for each corresponding term.

We note that $\frac{g_j}{{\Vert g \Vert}_2}\leq x_j$ is equivalent to $\frac{{g_j}^2}{{\Vert g \Vert}_{2}^{2}} \leq {x_j}^2$, so for each $j<i$ we have ${g_j}^2 \leq {x_j}^2 {g_j}^2 + {x_j}^2 ({g_1}^2 + ... + {g_{i-1}}^2 + {g_{i+1}}^2 +...+{g_{n}}^2  ) $, which can be rewrite as $ {g_i}^2 \geq \frac{{g_j}^2}{{x_j}^2} - ({g_1}^2 + ... + {g_{i-1}}^2 + {g_{i+1}}^2 +...+{g_{n}}^2  ) $. We can also write from $\frac{g_i}{{\Vert g \Vert}_2}\leq x_i$ and derive $ {g_i}^2 \leq \frac{{x_i}^2}{(1-{x_i}^2)} ({g_1}^2 + ... + {g_{i-1}}^2 + {g_{i+1}}^2 +...+{g_{n}}^2  )  $.

Therefore, $P(\frac{g_i}{{\Vert g \Vert}_2}\leq x_i \vert \bigcap_{j=1}^{i-1} (\frac{g_j}{{\Vert g \Vert}_2}\leq x_j) ) = P({g_i}^2 \leq \frac{{x_i}^2}{(1-{x_i}^2)} ({g_1}^2 + ... + {g_{i-1}}^2 + {g_{i+1}}^2 +...+{g_{n}}^2  ) \vert \bigcap_{j=1}^{i-1} ( {g_i}^2 \geq \frac{{g_j}^2}{{x_j}^2} - ({g_1}^2 + ... + {g_{i-1}}^2 + {g_{i+1}}^2 +...+{g_{n}}^2  ) )  ) \leq  P({g_i}^2 \leq \frac{{x_i}^2}{(1-{x_i}^2)} ({g_1}^2 + ... + {g_{i-1}}^2 + {g_{i+1}}^2 +...+{g_{n}}^2  )) = P(\frac{g_i}{{\Vert g \Vert}_2 }\leq x_i) $, which finished our proof of negative dependence. 






\begin{thm} [Strong Concentration] \label{Thm_StrongConcentration}

Suppose function $f: \mathcal{R}^{+} \mapsto \mathcal{R}$ can be decomposed as $f=f^{+} + f^{-}$, where $f^{+}$ and $f^{-}$ represent monotone increasing and decreasing part respectively. If $f^{+}(\vert \omega_i^T Z \vert) \in [a_i^{+},b_i^{+}]$ and $f^{-}(\vert \omega_i^T Z \vert) \in [a_i^{-},b_i^{-}]$ a.s., then $\hat{F}_m^{ort}(Z)=\frac{1}{m}\sum_{i=1}^m f(\vert {\omega_i^{ort}}^T Z \vert)$ satisfies upper tail bound:
$P(|\hat{F}_m^{ort}(Z) - F_f(Z)| \geq t)
 \leq 2\exp(-\frac{m^2 t^2}{2\sum_i {(b_i^{+}-a_i^{+})}^2})+2\exp(-\frac{m^2 t^2}{2\sum_i{(b_i^{-}-a_i^{-})}^2})$ a.s.. Furthermore, if $f$ is non-negative and monotone increasing (or decreasing), then orthogonal random features will provide tighter strong concentration bound than i.i.d random features: $P(\hat{F}_m^{ort} \geq a) \leq P(\hat{F}_m^{iid} \geq a)$, $P(\hat{F}_m^{ort} \leq a) \leq P(\hat{F}_m^{iid} \leq a)$, $\forall a>0$.
 


\end{thm}

Firstly, we decompose the estimator into increasing and decreasing parts: $\hat{F}_m^{ort}(Z) = \frac{1}{m} \sum_{i=1}^m f(|{\omega_i^{ort}}^T Z|) = \frac{1}{m}
\sum_{i=1}^m (f^{+}(|{\omega_i^{ort}}^T Z|)+ f^{-}(|{\omega_i^{ort}}^T Z|)) = {\hat{F}_m^{+,ort}}(Z)+{\hat{F}_m^{-,ort}}(Z)$, which are ND respectively. By applying Chernoff–Hoeffding inequalities for ND random variables \cite{Dev196}, we have:
$P(|\hat{F}_m^{+,ort}(Z) - F_{f^{+}}(Z)| \geq t)\leq 
2\exp(-\frac{m^2 t^2}{2\sum_i {(b_i^{+}-a_i^{+})}^2})$,
 $P(|\hat{F}_m^{-,ort}(Z) - F_{f^{-}}(Z)| \geq t) \leq 
2\exp(-\frac{m^2 t^2}{2\sum_i {(b_i^{-}-a_i^{-})}^2})$ a.s.. 
Therefore, $P(|\hat{F}_m^{ort}(Z) - F_f(Z)| \geq t) = P(|\hat{F}_m^{+,ort}(Z)+\hat{F}_m^{-,ort}(Z) - F_{f^{+}}(Z)-F_{f^{-}}(Z)| \geq t)
 \leq P(|\hat{F}_m^{+,ort}(Z) - F_{f^{+}}(Z)| + |\hat{F}_m^{-,ort}(Z)-F_{f^{-}}(Z)| \geq t) \leq P(|\hat{F}_m^{+,ort}(Z) - F_{f^{+}}(Z)|\geq \frac{t}{2})+ P(|\hat{F}_m^{-,ort}(Z) - F_{f^{-}}(Z)|\geq \frac{t}{2}) \leq 2\exp(-\frac{m^2 t^2}{2\sum_i {(b_i^{+}-a_i^{+})}^2})+2\exp(-\frac{m^2 t^2}{2\sum_i{(b_i^{-}-a_i^{-})}^2})$ a.s..


From Lemma \ref{Lem_NA_ExpectationProductInequality}, Lemma \ref{Lem_ND_2points} and Lemma \ref{Lem_abs_ort}, we can derive directly that if the function $f$ is monotone increasing (or decreasing) in $\vert \omega_i^T Z \vert$, then ND of $\vert{\omega_1^{ort}}^T Z\vert,...,\vert{\omega_n^{ort}}^T Z\vert$ implies $E[\exp(\lambda \sum_{i=1}^m X_i^{ort})] \leq \prod_{i=1}^m E[e^{\lambda X_i^{ort}}] = \prod_{i=1}^m E[e^{\lambda X_i^{iid}}] $, $\forall \lambda \in \mathcal{R}$, which is exactly the inequality for proving orthogonal random features have better strong concentration bound than independent random features derived after Lemma \ref{Lem_ExtendedMarkovInequality}.

==> conclusion.tex <==
\section{Conclusion}

We presented first general theory for the prominent class of orthogonal Monte Carlo (OMC) estimators (used on a regular basis for variance reduction), by discovering an intriguing connection with the theory of negatively dependent random variables. In particular, we give first results for general nonlinear mappings and for \textbf{all} RBF kernels. Inspired by developed theory, we also propose new Monte Carlo algorithm based on near-orthogonal samples (NOMC) that outperforms previous SOTA in the notorious setting, where number of required samples exceeds data dimensionality.

==> extra.tex <==
\subsection{Maximize angular among vectors}

Another way to construct almost orthogonal vectors is to avoid the sampled directions accidentally forming tiny angles. To address this issue, we propose a new estimator based on the $i.i.d.$ estimator. Instead of sampling $\omega_i$ independently, we would like  maximum angles to form among them. If we regard each direction as a particle on $S^{d-1}$, then it is equivalent to maximizing the distances between the particles. In practice, we define an energy function with respect to the distance between each pair of particles, which becomes larger and larger as the two particles approach each other. Then we use gradient descent method to minimize the sum of the energy of each pair while constraining the particles on $S^{d-1}$. We believe that the maximum angles will be roughly achieve after several iterations. To confirm our conjecture, we will show the visualization of the sampled directions in the next section with applications on Sliced Wasserstein distance. 

The energy between two particles $i$ and $j$ is assumed to be of the form: $E[\omega_i,\omega_j]=\frac{\delta}{\delta + {\vert \omega_i - \omega_j \vert}^2}$ for some $\omega>0$, so it decreases monotonically with respect to the distance between particles $i$ and $j$, therefore the force between them is repulsive. This minimization can be done by gradient descent. In the gradient descent, we had some work to do in order to find the right hyper-parameters for the optimization process. Indeed, we ran several instances of the algorithm with different number of directions to compute. Based on this study, we could conclude that for a fixed number of iterations in the gradient descent, a learning rate proportional to $\eta_t \sim \mathcal{O}(\frac{1}{N^\gamma})$. Where we empirically computed the optimal $\gamma=1$, and the multiplying factor to be 2. So the optimal leaning rate is $\eta_t =\frac{2}{N}$.


\subsection{Fixed construction for almost orthogonal vectors}

Another way to construct almost orthogonal vectors in the case $n>d$ is to set some fixed sequences to $\omega_i$'s. For example, we can pick the positive and negative axis of each dimension in $R^n$ to get $2n$ vectors, which are kind of evenly distributed in the space. Besides, we can also set our goal here to minimize $\varepsilon$ in $\vert \omega_i^T \omega_j \vert \leq \varepsilon, \forall i\neq j $, which can also be stated as the cross-correlation between different sequences. Actually, there has already been extensive research in the area of spread spectrum communication, which deals with the problem to minimize such cross-correlation as well as maximize linear complexity. Next, we will use the notation $(d,n,\theta)$ to represent a sequence set containing n sequences with period $d$, where the normalized absolute value of cross-correlations of each pair of sequences in this set is no greater than $\theta$. 

Gold \yrcite{Gold167} provided a construction for binary $\{+1,-1\}$ sequences using properties from $GF(2^m)$ and achieved $(d,2d,\frac{2\sqrt{1+d}+1}{d} \in \mathcal{O}(\frac{1}{\sqrt{d}}))$, where $d=2^m-1,  m\in \mathcal{N^{+}}$. Follow his definition, we denote $V(f)$ as the vector space of linear sequences generated by the recursion relation corresponding to the polynomial $f$ of degree $n$, which contains $d=2^n-1$ sequences with correlation equals exactly to -1. From Theorem 2 in Gold, let $f_1$ be the minimal polynomial of $\alpha$ and $f_t$ be the minimal polynomial of $\alpha^t$ where $t=\frac{\sqrt{4(1+d)}+1}{d}$ for $n$ even and $t=\frac{\sqrt{2(1+d)}+1}{d}$ for $n$ odd. Then $\alpha \in V(f_1)$ and $\beta \in V(f_t)$ implies $\vert \theta (\alpha,\beta) \vert \leq t$. Therefore, the maximum values of auto-correlation and cross-correlation values satisfies $\theta \approx \frac{1}{\sqrt{d}}$.




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



\section{Wasserstein distance and close-to-orthogonal sampling}

\subsection{Wasserstein distance}
In the last 3 years, the popularity of the Wasserstein distance has exploded in the field of data science, especially for generative models. It compares distribution with a global and geometrical approach, unlike point-wise metrics like the total variation.

For $p \geq 1$, the $p$-th Wasserstein distance between two distributions $\eta$ and $\mu$ over $\mathbb{R}^d$ is defined as:

$$W_p(\eta,\mu) = \left(\inf_{\gamma \in \Gamma(\eta,\mu)} \int_{\mathbb{R}^d \times \mathbb{R}^d} ||x-y||_{2}^{p} d\gamma(x,y) \right)^{{\frac{1}{p}}}$$

where $\Gamma(\eta,\mu)$ is the set of joint distributions over $\mathbb{R}^d \times \mathbb{R}^d$ for which the marginal of the first $d$ coordinates is $\eta$ and for the marginal of the last $d$ coordinates is $\mu$.

In particular, for point-cloud distributions $\eta= \frac{1}{M} \sum_{m=1}^{M} \delta_{x_m}$, and $\mu= \frac{1}{M} \sum_{m=1}^{M} \delta_{y_m}$, the Wasserstein distance can be written as:

$$W_p(\eta,\mu) = \left( \frac{1}{M} \sum_{m=1}^{M} \left|  x_i - y_{\sigma^*(i)} \right|^{p}  \right)^{{\frac{1}{p}}}$$

where the permutation $\sigma^*$ is an optimal assignment (not necessarily unique) that minimizes the sum of distances between the data points from $\eta$ and the data points from $\mu$ : 
$$\sigma^* \in  \underset{\sigma \in S_M}{\arg\min} \sum_{m=1}^{M} \left|  x_i - y_{\sigma^*(i)} \right|^{p}    $$

\subsection{Sliced Wasserstein distance}

Since the dimensionality for most of modern machine learning models can reach hundreds, the computation of the Wasserstein distance becomes a challenging problem. This is why the Sliced Wasserstein distance becomes more and more popular. It is a metrics that has the same purpose as the Wasserstein distance that uses projections of distributions in 1-D, to make the computation much faster.

The $p$-th Sliced Wasserstein distance is defined as:

$$  SW_p(\eta,\mu) = \left(   \mathbb{E}_{u \sim Unif(S^{d-1})} [W_{p}^{p}(\eta_u,\mu_u)]   \right)^{{\frac{1}{p}}}  $$

where $\eta_u$ and $\mu_u$ are the projections of $\eta$ and $\mu$ in the direction $u$. 

In most cases, the number of Monte Carlo simulations to compute the expected value in the formula of the Sliced Wasserstein distance has to be greater than the dimension ($N>d$). This makes it impossible to have $N$ samples $(u_n)_{n=1}^{N}$ that are perfectly orthogonal. For such cases, we have compared three different estimators of $SW_p$: an estimator using iid sampling (fig. \ref{visual}, a), an estimator using independant sub-families of $d$ orthogonal samples (fig. \ref{visual}, b), and an estimator using a pre-built set of close-to-orthogonal samples that maximizes the angles between each direction (fig. \ref{visual} c).



\begin{figure}[h]
\begin{subfigure}[t]{0.31\textwidth}
\centering
\includegraphics[scale=0.26]{IID.pdf}
\caption{i.i.d directions}
\end{subfigure}%
~
\begin{subfigure}[t]{0.31\textwidth}
\centering
\includegraphics[scale=0.26]{GS.pdf}
\caption{Independant sub-families of orthogonal directions}
\end{subfigure}
~
\begin{subfigure}[t]{0.31\textwidth}
\centering
\includegraphics[scale=0.26]{MA.pdf}
\caption{Maximum angles directions}
\end{subfigure}
\centering
\caption{Visualization of directions for d=3}
\label{visual}
\end{figure}

\subsection{Comparison of i.i.d v.s. close-to-orthogonal estimators}

We numerically compared the three above mentioned estimators of the SWD. As an illustration we choose $d=3$, which is convenient as we want to visualize the directions different estimators have sampled.

We know the analytical results for the 2-Wasserstein distance between Gaussian distributions, see for example Fig\ref{WikiAnalytical}.
\begin{figure}[h]
\centering
\includegraphics[scale=0.25]{AnalyticalGaussian.png}
\caption{2-Wasserstein distance for Gaussian distributions\\ \small{\url{https://en.wikipedia.org/wiki/Wasserstein_metric#Normal_distributions}}}
\label{WikiAnalytical}
\end{figure}

The closed-form formula for the 2-Wasserstein distance for Gaussian distributions enables us to get the closed-form formula of the 2-Sliced Wasserstein distance by computing the expected value. Thus, we have the exact value of the Sliced Wasserstein distance that we are trying to estimate, which enables us to compare the errors.

So, we assume, to illustrate our approach, that $p=2$, and that $\eta$ and $\mu$ are both Gaussian. In particular, we assume $\eta\sim\mathcal N\left(
\begin{bmatrix}
0\\
0\\
0
\end{bmatrix},
\begin{bmatrix}
2 & -1 & 0\\
-1 & 2 & -1\\
0 & -1 & 2
\end{bmatrix}
\right)
$
and
$\mu\sim\mathcal N\left(
\begin{bmatrix}
1\\
0\\
0
\end{bmatrix},
\begin{bmatrix}
3 & 2 & 1\\
2 & 4 & 0\\
1 & 0 & 2
\end{bmatrix}
\right)$.

Since we use point masses to discretize Gaussian distributions, we need to sample as many points as possible to reduce the truncation error. In our experiments, we let the number of points be $M=10^6$. We choose $N$, which is the number of directions, to be $40, 80, 120, 160, 200$, and we expect the estimators to be more and more accurate as $N$ increases.

For $N=200$, the directions sampled by the three estimators are shown in Fig \ref{visual}, where each red particle correspond a blue particle on the opposite position, and each pair of them represent one direction sampled. We can see that the directions sampled by i.i.d. and orthogonal estimators are heterogeneous, while those by maximum angular estimator seem to be homogeneous. Consequently, we won't be surprised if we find out the latter is of smaller variance. However, the homogeneity comes at a cost, since we have to compute the repulsive force between each pair of particles, so the computational complexity is $N^2$, while those for i.i.d. and orthogonal estimators are $N$ and $Nd^2$, respectively. Therefore, sampling processes by maximum angular estimator is relatively slow.

To compare the accuracy of the three estimators, we plot the average error versus $N$, as shown in Fig \ref{errorComparison}. We can see that the orthogonal estimator is slightly better than i.i.d. one, and that the maximum angular estimator is significantly more accurate than the others.
Still, there is a limit in our approach, as we used rather homogeneous distributions, gaussian distributions, it would be interesting to see how they perform with more complex distribution. Also, a future endeavor we would have tried with more time: if we can sample from each of the distributions, it could be interesting to consider sampling the directions according to the distribution, this way we could maximize the information gathered on the distributions at each iteration.

\begin{figure}[h]
\centering
\includegraphics[scale=0.7]{error.pdf}
\caption{Numerical performance of three estimators}
\label{errorComparison}
\end{figure}


\section{Application of theorem 1 : orthogonal features for kernel ridge regression}
\subsection{Problem Statement}
In this section, we consider random feature based kernel methods
on downstream tasks such as kernel ridge regression.
In this context, we assume that the training data $(x_1,y_1),...,(x_n,y_n)\in \mathcal{X}\times \mathcal{Y}$ satisfies:
\begin{equation*}
    y_i=f^*(x_i)+\nu_i
\end{equation*}
where $f^*$ is the groundtruth function to be learned and $\nu_i$ is iid noise.\\
The response KRR estimator for a given input $x$ is estimated as:
$$\bar{f}=\sum_{j=1}^{n}k(x_j,x)\alpha_j$$
where $\alpha = (\alpha_1, \cdots, \alpha_n)^T$
is the solution of the equation
$$(K + \lambda I_n)\alpha = y.$$
In the above, $K \in \mathbb{R}^{n\times n}$
is the kernel matrix given by $K_{ij} = k(x_i
, x_j)$ and $y =[y_1, \cdots, y_n]^T$
is the vector of responses.

Random Fourier features is an approach to scaling up kernel methods for shift-invariant kernels, which are kernels of the form $k(x,z)=k(x-z)$ where $k(\cdot)$ is a positive definite function (we abuse notation by using $k$ to denote both the kernel and the defining positive definite function but this can be easily understood from the context). The underlying observation behind random Fourier features is a simple consequence of Bochner’s Theorem: for every shift-invariant kernel for which $k(0) = 1$ there is a probability measure $\mu_k(\cdot)$ and
possibly a corresponding probability density function $p_k(\cdot)$, both on $\mathbb{R}^d$, such that
\begin{align}
k(x,z)&=\int_{R^d}\exp(-2\pi i \eta^T(x-z))d\mu_k(\eta) \\
&=\int_{R^d}\exp(-2\pi i\eta^T(x-z))p_k(\eta)d\eta.
\end{align}


\begin{thm}
Consider any shift invariant kernel $k$. Let $\hat{\Delta}$ denote the smallest positive number such that $\hat{K} + \lambda I_n$ is a
$\Delta$-approximation of $\hat{K} + \lambda I_n$, where $\hat{K}$ is an approximate
kernel matrix obtained by using an orthogonal random feature map based kernel estimator. Then for any $a > 0$:
\begin{equation*}
   \mathbb{P}[\hat{\Delta} > a]\leq N^2e^{-C m\frac{a^2\sigma_{min} ^2}{N^2}} 
\end{equation*}

where m is the number of features used, $C>0$ is a universal constant, N is the size of the dataset and $\sigma_{min}$ is the smallest eigenvalue of $K + \lambda I_n$
\end{thm}

\textit{Proof.}\\
The beginning of the proof is identical to the proof of Theorem 2 in \cite{CCB}, but we provide a much simpler proof of the following lemma. Furthermore, we extend it to the case of any RBF kernel, whereas only smooth RBF kernels were previously handled in \cite{CCB} (smooths RBF kernels have some additional conditions on their k-th moments).
\begin{lem}
Fix some $z\in\mathbb{R}$. For a sample $(w_1^{ort}, ..., w_m^{ort})$ from the continuous orthogonal distribution, the following holds:
\begin{equation*}
\mathbb{P}\left(\sum_{i=1}^m \tfrac{1}{m}(cos(w_i^{ort})^Tz-\phi(z)\right)>x\)\leq e^{-Cmx^2}
\end{equation*}
\end{lem}

This last inequality is a corollary from theorem 1. Indeed, we can write the cosine function as the sum of a nonnincreasing and a nondecreasing part: $\forall x\in [0,2\pi], cos(x)=f(x)+g(x)$ with $f(x)=1+\int_0^x max(0,sint(t)dt$ and $g(x)=\int_0^x min(sin(t)dt)$ and $||f||_{\infty}\leq 2\pi$, $||g||_{\infty}\leq 2\pi$.
